Investigating the efficacy of music version retrieval systems for setlist identification

The setlist identification (SLI) task addresses a music recognition use case where the goal is to retrieve the metadata and timestamps for all the tracks played in live music events. Due to various musical and non-musical changes in live performances, developing automatic SLI systems is still a challenging task that, despite its industrial relevance, has been under-explored in the academic literature. In this paper, we propose an end-to-end workflow that identifies relevant metadata and timestamps of live music performances using a version identification system. We compare 3 of such systems to investigate their suitability for this particular task. For developing and evaluating SLI systems, we also contribute a new dataset that contains 99.5h of concerts with annotated metadata and timestamps, along with the corresponding reference set. The dataset is categorized by audio qualities and genres to analyze the performance of SLI systems in different use cases. Our approach can identify 68% of the annotated segments, with values ranging from 35% to 77% based on the genre. Finally, we evaluate our approach against a database of 56.8k songs to illustrate the effect of expanding the reference set, where we can still identify 56% of the annotated segments.

==> old_introduction_v1.tex <==
\section{Introduction}
\label{sec:intro}
%\textit{Music recognition} term is commonly used in the academic and industrial world in order to refer to the task of identifying the presence of a known music track in an unknown audio stream\cite{Wang2003}\cite{Arcas2017}. In some contexts, other terms have been used to refer to the same task, such as \textit{music identification}\footnote{www.bmat.com}, or \textit{automatic content recognition}\footnote{www.acrcloud.com}. The broader sense of music recognition task aims at identifying not only the metadata of the music track used in an unknown audio stream, but also the exact start and end timestamps for each of them.

Music recognition is commonly used to refer to the task of identifying the presence of a known music track in an unknown audio stream, ideally along with its start and end timestamps~\cite{Wang2006a,Arcas2017}. The main applications of music recognition systems include music discovery for end users (e.g., Shazam and Soundhound) and copyright management for the music industry.
%Already being adopted by many agents of the music industry, the automatic MR systems attract a growing interest due to their continuously improved capabilities and benefits.\footnote{https://www.bmat.com/bmat-clients/}\footnote{https://www.audiblemagic.com/newsroom/blog/}
%\footnote{https://www.acrcloud.com/pros-labels/}\footnote{https://www.digitalmusicnews.com/2018/07/08/music-recognition-technology-mrt-2019/}\footnote{https://rightshub.net/music-recognition-technology-the-hidden-superpower-behind-the-worlds-leading-music-companies/}. 
The enormous variety of music usage contexts, which has increased significantly in the last years due to user-created materials in digital platforms, makes impossible to track music usage without automatic processes and, therefore, highlights the necessity of automatic systems. Moreover, in terms of copyright management, these technologies can be considered a game changer, since they allow to fairly distribute significant amounts of revenues to music creators\footnote{\url{https://www.toptal.com/finance/market-research-analysts/state-of-music-industry}} with a transparency that can not be achieved with previous manual workflows. \joan{I find this intro too focused on copyright management. We should be a bit more generic.}
 
 %Some examples of these applications are: broadcast music monitoring, venues music monitoring, setlist generation from full concerts, music catalog deduplication, shazam-like apps, copyright infringements detection of audio uploaded to digital platforms, etc. 

%Music copyright management mainly concerns two types of copyrights of a song\footnote{https://www.copyright.gov/circs/circ56a.pdf}, and understanding the distinction between them helps with choosing the correct technology for particular application scenarios. On the one hand, the Sound Recording Copyright is linked to a specific master recording, and typically managed by record labels. Audio fingerprinting systems\cite{Cano2005} are designed to handle this type of copyright by allowing to efficiently identify known recordings in the monitored audio streams. Although such systems can be robust to a number of audio degradations (e.g., voiceovers\cite{Wang2003}, pitch shifting\cite{Joren2014}, background noise), in cases where the original master recording is not present, their identification capabilities are severely impaired. On the other hand, the Songwriting Copyright is linked to the written song itself, and typically managed by publishers. The suitable technology for this case is the version identification systems that go beyond the near-exact duplicate detection to identify recordings that, although having perceptual differences, convey the same musical entity (e.g., live performances, cover songs). 

%Such systems are more suitable for the Songwriting Copyright management due to their goal of identifying various recordings that are derived from the same underlying composition.


%Audio fingerprinting is one of the most common music identification technologies [refs], and it allows to efficiently identify the usage of known master recordings in unknown audio streams. In some approaches, some common degradations of audio can be supported: voiceovers, usage of short audio excerpts, pitch-shifting[panako], microphone recordings, etc. However, audio fingerprinting approaches are not useful for cases where a music work is used, but the original master recording is not present at all, like in the case of live performances (e.g. full concerts, short live performances in TV shows, etc.), or in releases of versions of a music work. In these situations, version identification methods [ref] are more suitable to properly identify the usage of an original music work.

The monitoring of live performances for copyright management stands as a challenging branch of music recognition. \joan{Does the application on copyright management change the objective of the task? Does the fact that it is for copyright infringement imply that there are gonna be other changes in the recordings?} \joan{I'd go more to the point, just introducing the task of set list identification from the very beginning, and then going to the next sentence. Then, in the following paragraphs, there are many things that will have already been said. I see not much value for a short ICASSP paper in trying to structure the different terminology around the problem...}
Live performances can incorporate many alterations from the studio recordings, including changes in tempo, structure, background noise, additional applause and banters, and so on. The goal is to identify metadata and start and end timestamps for each individual song played in live music events (i.e., festivals, music venues). While the most common and successful technologies for music recognition are audio fingerprinting systems~\cite{Cano2005} that can identify known recordings albeit incorporating a number of slight audio degradations (e.g.,~background noise~\cite{Haitsma2001}, voiceovers~\cite{Wang2003}, or pitch shifting~\cite{Fenet2011a, Joren2014, Sonnleitner2014}), live performance monitoring typically requires version identification (VI) systems that are designed to go beyond the near-exact duplicate detection to identify recordings that, although having perceptual differences, convey the same musical entity (e.g.,~live performances or cover songs)~\cite{serra2009, bertin2012, doras2019, yesiler2020a, yesiler2020b}.

In the music information retrieval community, live performance monitoring is addressed by the live version identification and the set list identification (SLI) tasks. \joan{In the previous paragraph you said the same but didn't mention SLI. Say it only once and with VI or VI+SLI.} While former systems focus on adopting fingerprinting-based methods to identify short queries of live performances~\cite{seetharaman2017}, the latter concern with retrieving the metadata and timestamps for the full live performances, making it a better proxy for live performance monitoring from a copyright management view. SLI is formally defined by Wang et al.~\cite{wang2014} and divided into two sequential sub-tasks: set list identification and song segmentation. To our knowledge, there has not been any other work specifically targeting SLI. \joan{Didn't Wang et al address it?}

%In Music Information Retrieval community, live performance monitoring is addressed by the live version identification and the set list identification (SLI) tasks. While the systems for the former focus on adopting fingerprinting-based methods to identify short queries of live performances~\cite{seetharaman2017}, the latter concerns with retrieving the metadata and timestamps for the full live performances, making it a better proxy for live performance monitoring from a copyright management view. SLI is formally defined by Wang et al.~\cite{wang2014} as having two sub-tasks: (1) set list identification, where the goal is to retrieve only the related metadata in the correct order, and (2) song segmentation, where the systems further process the retrieved items to obtain correct timestamps. To our knowledge, there has not been any other work specifically targeting SLI.

The system proposed by Wang et al.~\cite{wang2014} starts with the assumption that the artist is known for each concert. For overlapping probe-excerpts, a VI system is used to return a set of candidate matches using thumbnails, and the final matches and their boundaries are identified among those candidates using a dynamic time warping algorithm. Finally, the evaluation of the system is performed on a dataset of 20~concerts from 10~rock bands, using 3~metrics: edit distance, boundary deviation, and frame accuracy. Although demonstrating a plausible performance, due to the computational complexities of the algorithms used in each step, scaling such system to reference databases of thousands of songs stands as a difficult challenge. \joan{There is only one system for SLI? Don't you think that because you use a narrow definition/terminology you're not excluding many other systems?}

\joan{Introduction up to here is too convolved. I'd rewrite it from scratch}

%The system proposed by Wang et al.~\cite{wang2014} assumes that the artist is known; therefore, the reference database for each concert consists of only the works of that particular artist. For overlapping probe-excerpts, a VI system is used to return a set of candidate matches using thumbnails, and the final matches and their boundaries are identified among those candidates using a dynamic time warping algorithm. Finally, the evaluation of the system is performed on a dataset of 20 concerts from 10 rock bands using 3 metrics: edit distance, to evaluate only the metadata information and order; boundary deviation, to evaluate the obtained timestamps of only the correctly-identified matches; and frame accuracy, to evaluate the percentage of correctly-identified frames for the entire concert. Although demonstrating a plausible performance, due to the computational complexities of the algorithms used in each step, scaling such system to reference databases of thousands of songs stands as a difficult challenge.

In this paper, we address the SLI task for investigating the efficacy of current VI systems in a wide range of use cases related to the monitoring of live performances. In order to mimic a realistic industrial scenario, our approach combines the previously-mentioned sub-tasks \joan{Which sub-tasks?} into a single task by creating an end-to-end workflow that takes audio signals as input and creates a final document with retrieved metadata and timestamps. By using fixed window and hop sizes, we compare the performances of three VI systems that produce overlapping matches that we further process to create the final results. We develop and evaluate our system using a newly-contributed dataset \joan{newly-contributed just means that someone contributed it, not that YOU are contributing it HERE} of 75~concerts that are categorized by varying audio quality and genres. We report our findings using 4~evaluation \joan{Always prevent breaking a line after a number of an abbreviation like Fig.~X} metrics following industrial practices. For reproducibility and enabling further research, we publish our dataset and evaluation code at \url{https://github.com/furkanyesiler/setlist_id}. 




%This paper addresses the problem of music monitoring of long live performances for automatic set list generation, i.e. providing metadata, start, and end times for each of the tracks played. In some cases, live performances are coming from a single known artist, so this extra information can be used to limit somehow the size of the catalog (typically to a few hundred tracks). Unfortunately, artist information is not available in many real-world situations, so the required catalog size typically ranges from hundreds of thousands of tracks (e.g. a collection of popular music tracks), to tens of millions of tracks in worst case. In the MIR community, the task commonly known as set list generation typically refers to the specific variant where artist information is available, so that we can significantly limit the catalog size. Some previous methods to address this problem are based on (...). More recent approaches (...). 

